Sentence Bottleneck Autoencoders from Transformer Language Models

Representation learning for text via pretraining a language model on a large corpus has become a standard starting point for building NLP systems. This approach stands in contrast to autoencoders, also trained on raw text, but with the objective of learning to encode each input as a vector that allows full reconstruction. Autoencoders are attractive because of their latent space structure and generative properties. We therefore explore the construction of a sentence-level autoencoder from a pretrained, frozen transformer language model. We adapt the masked language modeling objective as a generative, denoising one, while only training a sentence bottleneck and a single-layer modified transformer decoder. We demonstrate that the sentence representations discovered by our model achieve better quality than previous methods that extract representations from pretrained transformers on text similarity tasks, style transfer (an example of controlled generation), and single-sentence classification tasks in the GLUE benchmark, while using fewer parameters than large pretrained models.

==> sections-old/0-abstract.tex <==

\begin{abstract} %  
Pretrained language models based on transformers have been shown to produce sub-optimal sentence representations for tasks requiring text similarity \cite{Reimers2019SentenceBERT}.
Previous methods that ameliorate this issue have introduced auxiliary sentence similarity objectives that rely on annotated data and compose sentence representations with non-parametric pooling that exhibits limited desirable properties and is specific to text similarity tasks.
To this end, we propose \textsc{Autobots}, a new class of text autoencoders with a sentence bottleneck derived from pretrained transformers on unlabeled data.
Our training objective is to to reconstruct sentences fully from a learned bottleneck representation as opposed to partially from variable-length representations in existing masked language modeling objectives.
We demonstrate that our resulting sentence representations outperform previous methods on text similarity tasks  and can also be used for controlled generation tasks such as style transfer.
Notably our method maintains the performance of the pretrained language model on other supervised  downstream tasks.
\nikos{new take on the abstract, please check. I tried to emphasize on the sentence BERT method to have a clear message about our goal of the paper. There are some nice points in the previous abstract that should probably be incorporated in the introduction but it would be crucial not to make big claims about pretraining in general since it would be hard to compete with big LM papers. }


%Methods for obtaining unsupervised language representations have gained much attention recently for their performance on downstream tasks, and have largely relied on partial reconstruction of the input though masked language modeling or next token prediction through language modeling. Autoencoders, trained on full reconstruction of the input through a single fixed length, bottlenecked representation, have not been extensively studied for pretraining sentence-level representations, especially with transformers.
%In this paper, we propose the \textit{Transformer Autoencoder} by converting the architecture of \citet{vaswani17} to an autoencoder that uses attention to bottleneck the input to a single, fixed vector from which the input can be fully reconstructed. Leveraging the encoder advancements of \citet{devlin-etal-2019-bert}, we introduce \textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, and demonstrate the significant performance of this novel pretraining objective in downstream classification, sentence representation, reconstruction, and controlled generation tasks.

\end{abstract}

% Autoencoders have 

% Unsupervised pretraining has gained much attention recently 
% We propose the transformer

% Methods for obtaining unsupervised language representations have gained much attention recently for their performance on downstream tasks, and have largely relied on partial reconstruction of the input though masked language modeling or next token prediction through language modelling.

% Text autoencoders obtain an unsupervised sentence-level representation by bottlenecking with reconstruction abilities, but largely rely on recurreence in the decoder.

% In this paper, we propose the \textit{Transformer Autoencoder} model by converting the architecture of \citet{vaswani17} to an autoencoder that uses attention to bottleneck the input to a single, fixed vector from which the input can be fully reconstructed. Leveraging the encoder advancements of \citet{devlin-etal-2019-bert}, we introduce textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, to demonstrate the performance of this novel pretraining objective in downstream classification, sentence representation, reconstruction, and controlled genration tasks.

% by leveraging the encoder advancements of \citet{devlin-etal-2019-bert} in a transformer auto


% effectively enriching the resulting sentence representations with reconstructive properties. Concretely, we introduce a context attention bottleneck after the original encoder, and a modify the decoder to perform full reconstruction of the input conditioned on the bottleneck representation.
 
% Currently langauge representat
% 
 

% VERSION 1:

% % to learn 
% % \textit{BERT isn't an autoencoder, but BARNEY is!}

% Autoencoders have gained much attention for their unsupervised ability to reduce variable length sequences to a single latent space with reconstruction capabilities, yet current architectures rely heavily on recurrence. Similar to autoencoders, current state-of-the-art pretrained transformer models produce variable-length token represenations by learning to partially reconstruct their input, yet rely on a special token to produce sentence representations for most downstream natural language understanding tasks requiring a single vector.


% % Current state-of-the-art pretrained language models produce variable-length token representations by learning to partially reconstruct the input, and rely on a special token to produce sentence representations for most downstream natural language understanding tasks requiring a single vector. 
% %\nikos{we may want to mention that it's not possible to produce the full sentence based on cls alone} 
% %\nikos{the token level representations are used for word-level tasks though, so we have to make sure we don't overclaim here.}

% In this paper, we propose the \textit{Transformer Autoencoder} model that results from  converting the architecture of \citet{vaswani17} to an autoencoder that projects the input to a single, fixed vector from which the input can be fully reconstructed, effectively enriching the resulting sentence representations with reconstructive properties. 
% Concretely, we introduce a context attention bottleneck after the original encoder, and a modify the decoder to perform full reconstruction of the input %(instead of partial) 
% conditioned on the bottleneck representation.
% %to the "encoder-decoder" layer in the decoder stacks.
% %
% %We preserve the parallelism in the original transformer by analyzing dot-product attention's decomposition in the many-to-one and one-to-many settings. \nikos{Not sure I fully get this point. }
% %
% %\textbf{TAE} can be pre-trained on unlabeled corpora to produce a single sequence-level representation. \nikos{this point could be skipped}

% % Lastly, we develop an example framework called \textbf{BARNEY} based on transformer autoencoders for pretraining akin to BERT \citet{devlin-etal-2019-bert}
% Lastly, we introduce \textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, which both leverages advancements of \citet{devlin-etal-2019-bert} and introduces a novel pretraining objective for transformers. We evaluate its sentence representations on downstream classification, reconstruction and controlled generation tasks.\footnote{Our code will be made available at [link]} 


% %, which stands for \textbf{B}idirectional \textbf{A}ggregated Transformer \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}. \nikos{is it ok if we skip the abbreviations until we decide the proper framing?}
% % and  we evaluate its sentence representations on downstream classification, reconstruction and controlled generation tasks.\footnote{Our code will be made available at [link]} 

==> sections-old/1-introduction.tex <==
{\color{red}TODOS
\begin{itemize}
    \item Nikos: Take a pass thorugh abstract, introduction, transformer autoencoders, and BARNEY sections for quick feedback/throughts/quick edits \nikos{done}
    \item Ivan: Finalize tables, experiments, and figures, then work on text
    \item Ivan $\&$ Nikos: Related Work \nikos{let's incorporate everything in the introduction. dedicating a whole section for this does not make much sense for a short paper.}
    \item Ivan: Implement Nikos's feedback and improve first draft
    \item Ivan: Shorten to 4 pages for EMNLP short paper submission
\end{itemize}
}

\section{Introduction} 
\nikos{need to convert to full text}
{\textit{Contributors}}: Ivan, Nikos, Noah

\vspace{3mm} 
\noindent \textit{Significance:} Recently, research has focused on devising new pretraining objectives for transformer-like architectures all involve some form of  language modeling (masked, generalized, etc) with much success for downstream tasks. Surprisingly, the direction of creating a complete autoencoder-like pretraining objective for transformers  still remains unexplored. We suspect this is mainly due to the variable-length nature of decoders in the original encoder-decoder transformer architecture by \citet{vaswani17}.

\begin{figure}[ht]
\centering
\hspace{-2mm}\includegraphics[width=0.5\textwidth]{figures/fig.png}
\caption{\ivan{TODO: Better quality diagram}\nikos{+1, I would keep it minimal and relatively small to save space e.g. even simpler than \url{https://paperswithcode.com/media/methods/Autoencoder_schema.png} perhaps with some indication that the encoder is a pretrained transformer.}}
% \caption{\label{fig:overview} We propose a novel task setup to multilingual question answering. A high resource language (HRL) question-answer database is leveraged by mapping a low resource language (LRL) query to a query in the database, then generating the LRL answer from the HRL answer.} % We examine using multilingual paraphrase detection in exploring the most reliable method to transfer knowledge from multilingual queries to English.
\end{figure}


\noindent \textit{Problem}:
\nikos{here we need also to highlight the issue that was identified for sentence representations extracted from BERT in the SBERT paper and cite several studies that focus on sentence representations. By the way, do we have any comparison with other methods than SBERT? In that paper, they compare with other methods. Could we also compare with those?}
Most pretrained language models rely on a special token to produce sentence representations for downstream classification tasks (BERT, ELECTRA) which does not guarantee perfect reconstruction of the input, a property that could be useful for tasks where autoencoders are useful such as controlled generation.
Moreover, they produce variable-length token representations which are often not needed for the downstream tasks and are potentially redundant. 
Additionally, during masked language modeling, only select tokens are updated each gradient step, encompassing wasted computation. To our knowledge, transformers decoders have not been explored in the context of a single encoder representation as input.
% \ivan{The [CLS] token, for BERT, is trained on the NSP task, which isn't sufficient for single-sentence representations. Additionally, in RoBERTa, they simply drop the NSP task altogether}

%\ivan{The two goals of this architecture: Improve BERT pretrained sentence representations, and provide a novel autoencoder (with better reconstruction properties)} 
\vspace{3mm} 

\noindent \textit{Questions}:
\begin{enumerate}
    \item Can we train BERT with a bottleneck representation from which the full input can be reconstructed?
    \item How well will such representations perform on different tasks compared to the [CLS] token from BERT?
    \item Will this autoencoder produce a latent representation that will do better on controlled generation tasks?
    \item Can we obtain better token representations from BERT when pretraining on both the MLM and reconstruction objective?
    %\item What do we want to make the scope of this paper be?
    %\item Will this autoencoder do well in multilingual settings?
\end{enumerate}

\vspace{3mm}

\noindent \textit{Method}
We introduce a context attention bottleneck for the encoder of \citet{vaswani17}, and an alternative decoder trained to perform full reconstruction of the input which is conditioned on the bottleneck representation.
As a use case we develop a language model pretraining framework based on our autoencoders akin to BERT. 

\vspace{3mm} 

\noindent \textit{Evaluation} We plan to evaluate on natural language understanding tasks from GLUE benchmark, on universal sentence representation tasks, and on autoencoder-related tasks related to reconstruction and  controlled generation such as style transfer or unconditional text generation. \nikos{let's make sure we include all the experimental details in the supplementary material (following emnlp guidelines) plus qualitative examples for all tasks that we examine.}
 %\ivan{Perhaps on reconstruction ability as well?}

% \textit{Plan:}
% \begin{enumerate}
%     \item Classification tasks: We will primarily look into the GLUE framework to see what improvements BARNEY offers over BERT for classification, and see (using NLI/STS) its performance at creating sentence representations.
%     \item Generation tasks: We will evaluate on the Shen et. al. task to evaluate the generation capabilities of BARNEY and how it does as an autoencoder.
% \end{enumerate}

% \\
% \ivan{TODO List: \begin{enumerate}
%     \item Discuss the method more
%     \item Show the tables we would like to express, and what results we want to see.
% \end{enumerate}}
%\section{Context}
% Attention is All You Need \\
% RNN Autoencoder: \\
% Can get metrics in a multilingual setting (LASER): https://arxiv.org/pdf/1812.10464.pdf \\
% BERT: \\

% Can evaluate on all the tasks for reconstruction in emb2emb, and add classification on top. Emb2emb already contains everyting needed to evaluate

% Tasks can be multilingual (use multilingual BERT, eval against LASER)


==> sections-old/2-transformerautoencoders.tex <==


\section{Proposed Method: \textsc{Autobots}}

\subsection{Encoder model}

\subsubsection{Pretrained transformers} 
\nikos{should also mention here the finetuning options} 

\subsubsection{Context Attention Bottleneck} 

\subsection{Decoder model}

\subsection{Training objective}




\nikos{I'd be in favor of merging the two sections below into one section with the structure above. Let's not overwhelm the reader with two proposed ideas. Let's keep it simple.}
\section{Transformer Autoencoders}
%\nikos{The two sections could probably be merged together to simply BARNEY, unless we decide to pitch it as "Transformer autoencoders for language understanding (Barney) and generation (emb2emb)."}
\nikos{this paragraph is a bit redundant. we could move it in the introduction.}
We describe here the proposed Transformer Autoencoders (TAEs). The main idea is to convert the encoder-decoder transformer architecture proposed by \citet{vaswani17} to an autoencoder architecture. The main difficulty we are addressing here is that the original encoder-decoder transformer operates with variable-length vectors. We show below how it can be adapted to work with a bottleneck using fixed-length vectors. The resulting autoencoder can be used for monolingual \cite{devlin-etal-2019-bert} pretraining, multilingual pretraining \cite{artetxe18} or it can be used for solving sequence-to-sequence tasks such as machine translation \citep{vaswani17}.=
%\nikos{By the way if this works we could even test it for translation in the future.} \ivan{Good point! I had ideas of using it with mBERT and possibly creating better language-agnostic representations, a similar setup to Facebook's LASER}
%- \url{https://arxiv.org/pdf/1812.10464.pdf} \\
% \ivan{I have some ideas for the MT idea (but probably shouldn't be in the scope of this paper)}

\subsection{Context Attention Bottleneck}
\nikos{see comment above}
The Transformer encoder architecture outputs a hidden representation $\mathbf{h_t}$ for each input token $x_t$. We wish to reduce these representations to a single, fixed representation $\mathbf{z}$. The self-attention layers used in Transformers produce a many-to-many representation by making the keys, queries, and values come from the same input. In order to produce a many-to-one final representation, we introduce a context vector $\mathbf{u}$ to replace the query. 
% \ivan{I commented out option (1), which we could explore later, option (2) boils down to multihead attention with nhead=1, which we can examine in an ablation study}
\begin{align*}
    \mathbf{z} &= \text{CAB}(\mathbf{u}, \mathbf{K}, \mathbf{V}) \\
    &= \text{MultiHead}(\mathbf{u}^\top, \mathbf{K}, \mathbf{V}) \\
       &= \text{Concat}(\text{head}_1, ..., \text{head}_n) \\%\mathbf{W_C} \nikos{is this transformation needed?}
      \text{head}_i = & \text{Attention}(\mathbf{u}^\top \mathbf{W^{(i)}_Q}, \mathbf{K} \mathbf{W^{(i)}_K}, \mathbf{V} \mathbf{W^{(i)}_V})
\end{align*} 
% As such, we explore the following options to compute the bottleneck representation \\

% \vspace{1mm}

% \noindent \textbf{Option 1:} Use an attention function akin to the one used for parametric pooling at different levels in hierarchical attention networks \cite{yang-etal-2016-hierarchical}
% %
% $$a_t = \frac{ \exp\big[{\mathbf{u} \cdot \sigma(\mathbf{W_a}  \mathbf{h_t} + \mathbf{b_a})}\big]}{\sum_{i=1}^T  \exp\big[{\mathbf{u} \cdot \sigma(\mathbf{W_a} \cdot \mathbf{h_i} + \mathbf{b_a})\big]}} $$
% $$\mathbf{z} = \sum_{t=1}^T a_t \cdot (\mathbf{h_t}  \mathbf{W_v})$$
% %
% where $\sigma(\cdot)$ is an activation function, here \textit{tanh} and $W_k$, $b_k$ are the parameters of the attention transformation.  

% \vspace{2mm}

% \noindent \textbf{Option 2:} Modify the dot-product self-attention used in transformers \cite{vaswani17} to be a learned-context attention, as follows
% %
% $$\mathbf{z} = \text{Attention}(\mathbf{u}^\top, \mathbf{K}, \mathbf{V}) = \text{softmax}(\frac{\mathbf{u}^\top \mathbf{K}^\top}{\sqrt{d_k}})\mathbf{V}$$
% %
% \noindent where the matrices $\mathbf{K}, \mathbf{V}$ correspond to the key  and the value matrices from the original transformer. Note that the query $\mathbf{Q}$ matrix is not used in the computation. \nikos{Instead of learning $\mathbf{u}$, couldn't we make use of $\mathbf{Q}$ by setting $u = \sum_j Q_j$?} \ivan{I like this idea too. Similar commentary as the [CLS] below}

% \vspace{2mm}

% \noindent\textbf{Option 3:} Extend option two above to a multi-head learned-context attention as follows
%

% \nikos{if we set u to [CLS] representation at the N-1 layer above do we recover the final [CLS] representation in BERT?}
% \ivan{That's actually a great idea/point, I think BARNEY should be the N+1th layer with [CLS] being it's u. We do recover it, but since our objective is different, it makes this method interesting}
% \ivan{That's really good suggestion/point! In the general case of the "learned context attention bottleneck", we can just say the context vector is learned, but in the BARNEY case, the context vector is just the [CLS] token. Perhaps our bottleneck should be called a "Context Attention Bottleneck" instead} \ivan{But to your question, it pretty much would, except for the fact that we're ramping up the amount of heads. Having $N_{head}$=$d_{model}$ is motivated by the fact that the gating mechanism is element-wise, and having that many heads will make the model do separate attention per element}
%
% where the number of heads $n$ can be \textit{large} ($n=d_{model}$), permitted by  the fact that the query is a single context vector. This allows significantly larger expressivity than the previous two options with comparable computational overhead as a single transformer layer.
The learned-context attention bottleneck module can be applied to the output of any transformer encoder architecture.

% \vspace{2mm}
% Of course, there are other  ways to define the bottleneck that does not require learning any parameters such as max-pooling or averaging with which we plan to compare in Section \ref{sec:experiments}
\noindent 
% \cite{Reimers2019SentenceBERT} explore non-parametric pooling bottlenecks such as max and averaging in addition to the [CLS] token of BERT, and we compare the performance of our method using their framework in Section \ref{sec:experiments}.

%\noindent \nikos{Would it make sense to learn a different u for different lengths of the context? e.g. sentence vs phrase, vs paragraph? By the way the learned context attention could be furthermore conditioned on other kinds of information in future work (e.g. sentiment). } 
%\ivan{That's a good point. Iteration 1 comes directly from the following paper: \url{https://www.aclweb.org/anthology/N16-1174.pdf}. Iteration 2 is pure decomposition of attention in the many-to-one case. Idea 3 (new!) is to use the context vector in Multihead Attention, and since the context is simply a single query vector, we can make the number of heads \textit{large}. It's a lot more expressive, and I like the phrase \textbf{BARNEY has \textit{many} heads}} \\\\

% \ivan{I'd like to test out this bottleneck against simple pooling methods, such as max/mean. I'd also like to see how gating does against no gating. Use to evaluate on the task? Just evaluate validation loss/BLEU?}
% \nikos{Good idea. We know from prior work that learned context attention is better than average (https://arxiv.org/pdf/1707.00896.pdf) but it would be nice to verify and compare with max pooling too. When you say gating you mean element-wise product with a learned vector + sigmoid? } \ivan{Yes! When I refer to "gating", I refer to the modifications to the "gating" solution in the decoder section} \nikos{Evaluating on validation loss makes sense but I am not sure we can afford training until convergence for each of these options. Perhaps, test validation scores for a fixed number of epochs? it's definitely not ideal but it could give us some initial clues. We should probably put more weight on the option 3 which is close to the way the [CLS] token is computed.   }
% \ivan{Very good point. I initially had the options to show the iterations from the initial bottleneck idea to a more expressive one (the multihead one). The SentenceBERT specifically aims at making sentence representations and explores max vs. mean vs. sum, and find that mean works best. I feel like focusing on just the multihead (option 3) would be best, and we can do an ablation study on the STS task for the amount of heads (and optionally options 1 and 2)}

\input{tables/glue}
\subsection{Encoder}
\nikos{see comment above}
Let $\text{TE}(x)$ be an arbitrary transformer encoder and $\text{CAB}(x)$ be the Context Attention Bottleneck specified above. Then, the encoder of our transformer autoencoder is defined as the following.
$$\mathbf{z} = \text{Enc}_{\text{TAE}}(\mathbf{x}) = \text{CAB}(\mathbf{u}, \text{TE}(\mathbf{x}), \text{TE}(\mathbf{x}))$$
The context vector $u$ can be either be represented as a learned parameter, or a pooling of the $\text{TE}(\mathbf{x})$. This context vector could additionally used to condition on different contexts to adapt a particular bottleneck to different types of information.
% An interesting property of the context attention is that the context vector can be specific to different types of contexts e.g. sentences or paragraphs. An extension would be to condition the attention function with other kinds of information (e.g. sentiment) as done in autoencoders for style transfer. 

% \nikos{We may want to optionally share the parameters of encoder and decoder for efficiency. }
\subsection{Decoder}
\nikos{see comment above}
The "encoder-decoder attention" layer in the Transformer decoder architecture by \citet{vaswani17}  expects hidden representations for every token input from the encoder in order for each output candidate to attend to each input token. In the situation where only a single representation comes from the encoder, we get the following:
% Analyzing the self attention in the context of \textbf{TAE}, both the memory keys and values in the self attention come from the single hidden representation $z$, which reduces to simply the linear transformation of the latent representation of the input sequence for each output candidate. \ivan{Using the notation in the original paper, the derivation would be the following:}
$$\text{Attention}(\mathbf{Q}, \mathbf{z}^\top \mathbf{W_K}, \mathbf{z}^\top \mathbf{W_V}) = \mathbf{z}^\top \mathbf{W_V}$$
Note that the queries Q, which come from the previous masked self-attention layer, aren't taken into account, and each step in the decoder will recieve the exact same $\mathbf{z}^\top \mathbf{W_V}$ as a result.  In order to mitigate this, we propose a gating method to allow the input query to control the per-element amount of information to include from the hidden representation vector. %\nikos{nice!}  
Concretely, let $\mathbf{Q_t}$ be the $t$-th query representation. Then, the $t$-th output $\mathbf{o_t}$ of the "encoder-decoder" layer will be the following:
$$\mathbf{g_t} = \sigma(\mathbf{W_{gh}}  \mathbf{Q_t} + \mathbf{W_{gz}}  \mathbf{z} +  \mathbf{b_g})$$
% \nikos{the gate $g_t$ doesn't look at the \mathbf{z} vector at all, so it's output will be independent of the z vector. we should probably add z as input to make sure features from both $h_t$ and $z_t$ are considered. e.g. $W_g h_t + b_g + W_z z + b_z$}
$$\mathbf{o_t} = \mathbf{g_t} \odot \mathbf{z}^\top\mathbf{W_V}$$
\noindent where $\sigma(\cdot)$ is the \textit{sigmoid} activation function and $\mathbf{W_g}$, $\mathbf{b_g}$ are the parameters of the transformation for the gate.
One can view the role of the gate here as determining how much information from the linear transformation of the latent representation to extract for the current layer and timestep.
% \ivan{Because of this per-element gating, I suspect that the case where $\text{nhead}=d_model$ in the context attention bottleneck will do best.}
% \ivan{Side thought: If the idea is to "extract" per element information from the hidden vector, should the bottleneck's objective be to "populate" per element information. Kinda like multihead attention where nheads=hidden size}

==> sections-old/3-barney.tex <==

\section{BARNEY} % Use case: Language Model Pretraining
\nikos{this first paragraph could be skipped, let's keep only the essential part the equation and the way the representations are selected from a pretrained model. would be good to start for Section 2}
The proposed autoencoder architecture can be used in tandem with any kind of transformer encoder network and can take advantage of pretrained language models such as BERT. In particular, we develop a new language model pretraining framework based on transformer autoencoders using BERT as an encoder function. Our framework is called \textbf{BARNEY} which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}. The final fixed-length representation which can be used for downstream tasks is thus computed as follows:
$$\text{Enc}_\text{BARNEY}(\mathbf{x})=\text{CAB}(\text{BERT}(\mathbf{x})_0, \text{BERT}(\mathbf{x})_{1:})$$
 
Particularly, we set the context vector $u$ equal to the representation of the $\text{[CLS]}$ token, tasking the $\text{[CLS]}$ representation with learning task-specific context. In effect, recovers the $\text{[CLS]}$ representation at the $N+1$th layer, fully utilizing the $N$th layer representations and reducing the unnecessary computation at the $N$th layer when utilizing only the $\text{[CLS]}$ token.

The amount of decoder layers depends on the targeted downstream task. For classification tasks, a shallow 1 layer decoder would emphasize better encoder representations. For generation tasks, more decoder layers are preferred to adequately model the language.

% If one's goal is to use BARNEY for encoding or classification tasks, one would choose a shallow 1 layer decoder to emphasize better encoder representations. Alternatively, if one wants to use the 
% \ivan{This addresses the wasted computation when just using [CLS]}
% And then a transformer decoder is trained on top.
\subsection{Training objective}
\ivan{TODO: Condense this section. The training methods (normal, denoising, MLM+denoising can be consolidated) }\nikos{+1, do we make use all of these options? denoising vs normal etc? make sure we keep only the ones that we actually experiment with.}
%\nikos{We should describe this in detail and discuss it because it deviates completely from the training objective of bert (masked language modeling, next sentence prediction). } \ivan{Good point!}
Unlike the masked language modeling and next sentence prediction pre-training objectives of BERT, we introduce the unsupervised reconstruction objective by pairing \textbf{BARNEY} with a transformer decoder and train on the task of reconstructing its own input. Below are the methods that consider both fixed and trainable BERT:

\subsubsection{Fixed BERT}
One can use the fixed weights from BERT, and only finetune the bottleneck of the encoder with the decoder. Inspired by the objective of preserving the BERT representations, this method experiences speed benefits from not needing to backpropogate into BERT. The two methods this can be applied to are the following:

\paragraph{Normal}
Pretraining on only the reconstruction objective when encoding and decoding the input.

\paragraph{Denoising}
Passing in corrupted input and training on the objective of reconstructing the original, non-corrupted input, as denoising has been shown to improve autoencoder representations. \citep{vincent2008denoising}


\subsubsection{Trainable BERT}
In pretraining and other uses, one can consider training BARNEY end-to-end with BERT being trainable. The main appeal of this method is if one was to start from scratch, 

\paragraph{Normal/Denoising}
Both of the above Normal and Denoising methods can be used with a trainable BERT.

\paragraph{MLM + Denoising}\nikos{is this objective used in the experiments or not?}
One concern is during \textbf{BARNEY} pretraining with trainable BERT is that the BERT final representations become saturated. This method aims to alleviate this problem by using the masked langauge modeling input as the "corrupted" input, and the masked language modeling objective will be used on top of the BERT representations during training in conjunction with the reconstruction objective. This method can be done from scratch; MLM only updates a handful of tokens in each gradient step, whereas the autoencoding objective takes into account \textit{all} token representations, therefore making greater use of a single backpopogation step and enriching the tokens with sentence-level information.

% \paragraph{Fixed BERT}

% Same as the Normal method, except o
% \paragraph{Denoising, Fixed BERT}
% Same as the Denoising method, except one would use the fixed weights from BERT \\


% The non-fixed BERT methods can also be considered when starting pretraining from scratch, but we will leave that study for further work due to computational restraints. 

% One concern is during \textbf{BARNEY} pretraining is that the BERT final representations become saturated. Additionally, it has been shown that the denoising improves autoencoder representations \citep{vincent2008denoising}. As such, we experiment with using the masked language modeling (MLM) input for the encoder during training. We test out having the MLM objective, to prevent saturating the original BERT representations, and without, to train \textbf{BARNEY} as a denoising autoencoder.
 
\subsection{Finetuning on downstream tasks} \nikos{this section could be condensed quite a bit and be described in the experiments section. note also that we don't focus on two-sentence tasks here, the sentence below about them could go into a footnote or in the supplementary.}

\paragraph{Classification} One can finetune a linear classification head on top of the \textbf{BARNEY} final representation, with all parameters finetunable. In the scenario where multiple sentences are given as input, one could either input both into the model to take advantage of cross attention, or encode the sentences separately and finetune a linear layer on a combination of the sentence representations.

% we experiment with inputting the two sentences into \textbf{BARNEY} versus encoding each sentence separately then finetuning a linear classification head on top of a combination of the features.
\paragraph{Sentence Representations} 
\citet{conneau2017supervised} show that one can obtain universal sentence representations by finetuning on natural language inference data. One encodes both sentences separately with BARNEY to obtain representations $u$ and $v$, then finetune a linear classifier on the $[u, v, |u-v|]$ concatenation of the representations.


\paragraph{Generation}
A generation task that requires generating a sentence from a single vector representation can easily take advantage of the transformer decoder


% \paragraph{Variable-Length Outputs} While not trained explicitly for this, one can evaluate the underlying BERT model. We suspect that the MLM + reconstruction would do best


% \ivan{For classification it would be simply putting a linear classification head on top of \textbf{BARNEY}, and finetuning to the given task. We might need to discuss ideas about tasks where two input sentences are given}
% \nikos{The main challenge is when we have tasks that involve multiple inputs e.g. entailment or question answering. In the BERT/GPT papers they tried to minimize task-specific modifications by serializing them with delimiters to process all of them as a single sentence. Eventually, they use [CLS] token embedding for the final classification. Not sure if doing the same with our model makes much sense though. It's going to be difficult avoiding task-specific modifications. Perhaps we could project them into the latent space separately and then add/multiply/concat them together to a fixed vector.} \ivan{That's a very good point. Given the overparameterization of BERT, I was thinking we could \textit{continue} with the MLM task in addition to the reconstruction objective (I explain it below)}


==> sections-old/4-experiments.tex <==

\section{Experiments}\label{sec:experiments}
Here, we present BARNEY finetuning performance on several different tasks. \nikos{we need to be more specific here. what are the questions we would like to answer specifically or our hypothesis. make sure the points we make correspond to the claims that we make in the intro/abstract and are clearly stated.}
For fair comparison, we pretrain \textbf{BARNEY} on the same Wikipedia + BooksCorpus dataset from BERT. To avoid training from scratch we use the pretrained BERT model as a starting point for our encoder function. We consider several different methods of pretraining. \nikos{these sound like experimental details, I would mention the basic ones in a subsection here and defer the rest for the supplementary (make sure we include everything there).}


% \subsection{BARNEY Pretraining for Classification}
% We outline several methods to pretrain BARNEY, and perform experiments on the sentence similarity task (SST2) with RoBERTa-base BARNEY, to observe the relative performance on single-sentence classification.

% \input{tables/barney_training_sst}

\noindent \textbf{Datasets} \nikos{Mention some basic details about the datasets used here.}
 
\noindent \textbf{Model configuration} \nikos{Only the basic ones and defer to the supplementary for the details such as number of epochs, learning rate etc. (e.g. we follow configuration from ...)}

\noindent \textbf{Baselines} \nikos{Describe our baselines and the versions of our model that we examined.}

\subsection{GLUE}
The General Language Understanding Evaluation (GLUE) benchmark \citep{wang2018glue} is a collection of diverse natural language understanding text classification tasks. We evaluate BARNEY pretrained with the Denoising, Fixed methodology report its performance on the dev set of each task in Table 1. \\
We find that on multiple tasks BARNEY on the base models end up performing on par with the large models with a mere fraction of additional parameters and compute. 

% \ivan{Since these are classification tasks, I feel like BARNEY would have a good chance at beating BERT as a baseline. These classification task require backpropagation through BARNEY, in addition to the linear classification layer, in the finetuning process.}
% \nikos{We should definitely try this. I am curious to see how the autoencoder pretraining objective impacts the results. } 



% \subsection{SentEval}
% SentEval [cite] is an evaluation framework for fixed sentence embeddings on 17 downstream tasks. We follow a setup similar to \cite{Reimers2019SentenceBERT} by finetuning on a combination of Natural Language Inference and Semantic Textual Similarity training sets, then finetuning a linear regression head on the fixed representations for each task. We examine the perfomrance of both BARNEY and BERT + CAB.
% % \ivan{These are 17 downstream tasks that \textit{don't} backpropagate through the sentence encoder, but rather, evaluate the fixed-length sentence embeddings themselves. \url{https://github.com/facebookresearch/SentEval}. If we include BERT's [CLS] token in this framework, we definitely have a good shot here}
% \nikos{I don't believe that this evaluation will measure the full potential of the method since it's best on fixed embeddings. By the way some of these tasks overlap with GLUE where we plan to test anyway with finetuning (e.g.SST/MRPC). So, I'd rather suggest to look for some controlled generation task such as sentiment style transfer (e.g. like the one used by Shen et al 2020) to demonstrate the benefits for a real  generation task (other than the reconstruction tests below).}
% % \ivan{Gotcha. In SentenceBERT they test the fixed embeddings after finetuning to the NLI dataset, which I feel like a good table to include would be an extra row for our method on table 5: \url{https://arxiv.org/pdf/1908.10084.pdf}}


\subsection{Sentence Representations}
\citet{Reimers2019SentenceBERT} perform the methodology of \citet{conneau2017supervised} of finetuning on NLI by using simple pooling methods of BERT representations, such as mean, max, and cls, and evaluate their performance on sentence similarity task. We train and evaluate BARNEY with a similar setup and its unique context attention bottleneck to compare against their results.
 
% \citet{conneau2017supervised} show that one can obtain universal sentence representations by finetuning on natural langauge inference data. \citet{Reimers2019SentenceBERT} show how this methodology can be applied to pooled BERT representations to obtain such sentence representations. We compaire

\input{tables/pooling}

We find that using the context attention bottleneck provides significant gains over using the other simple pooling methods. We suspect is due to the bottleneck acting as "weighted pooling" by attending over all the final tokens, to compute the final representation rather than mean/max equally considering all tokens or cls considering the representations before the final layer.

\input{tables/sts}

Using this setup, we compare directly the performance of BARNEY to other models on the sentence similarity task, ones which have not been trained on STS data. We find that BARNEY ends up performing singificantly better, and ends up achieving SBERT-large level performance with significantly less parameters.


% \subsection{BARNEY Pretraining for Generation}
% We outline several methods to pretrain BARNEY, and perform experiments on the sentence similarity task (SST2) with RoBERTa-base BARNEY, to observe the relative performance on single-sentence classification.


\subsection{Unsupervised Style Transfer}
% sentiment style transfer (e.g. like the one used by Shen et al 2020)
To evaluate properties of the latent space of BARNEY, we perform the experiment of \citet{shen2019educating} were we compute a “sentiment vector” $v$ from 100 negative and positive sentences, and change the sentiment of a sentence by encoding it, adding a multiple of the sentiment vector to the sentence representation, then decoding the resulting representation. We observe how the accuracy, BLEU, and perplexity change as we add a larger multiple of the sentiment vector to the representation in Table 4.

% and use it to change the sentiment of the test sentences.

\input{tables/generation}

% \subsection{Reconstruction Quality}
% \ivan{Perhaps we should evaluate the reconstruction ability compared to other autoencoders? We could focus on just BooksCorpus, create our own test set, and test reconstruction quality. If TAE/BARNEY is really good, we could introduce EM as a metric}
% \nikos{ What do you mean by EM? I worry that we may not have the space for introducing a new evaluation too (we have new architecture + pretraining framework already). How about using the Yelp dataset to compare directly with Shen et al 2020 in their own setup? }


% \subsection{Latent Properties}
% \ivan{We could also show an example of encoding two sentences, then showing the decoding of the linear interpolation of between the two? Perhaps a 2D dim-red of the embeddings?} \nikos{Sure, that'd be great. E.g. like the ones here \url{https://arxiv.org/pdf/1511.06349.pdf}}



% \subsection{Multilingual}

% \subsection{Pretraining}
% \begin{itemize}
%     \item Train two models on the exact same data for the exact same amount of training steps. To simulate the same amount of parameters, use one extra layer for the MLM approach
%     \item Model 1: 7 layer, 512 hidden size transformer encoder trained on just the MLM objective
%     \item Model 2: 6 layer, 512 hidden size BARNEY trained on MLM objective in conjunction with reconstruction objective.
%     \item Show the down-stream MNLI performance difference after certain amounts of steps (could be a plot)
%     \item Show the downstream SQuAD (MNLI?) performance difference at the end of BARNEY wihtout the conetext attention bottleneck (see if the reconstruction objective helps with better token-level representations, since all tokens are updated each step, rather than only 15\% of them in MLM)
% \end{itemize}

==> sections-old/5-ablationstudy.tex <==
\section{Ablation Study}


\subsection{Autoencoding Steps}

\input{tables/pretraining_steps}

\subsection{Finetunable BERT Layers}

\input{tables/finetunable_layers}



% \section{Ablation Study}
% We outline several methods to pretrain BARNEY, and perform experiments on the sentence similarity task (SST2) and reconstruction objective with RoBERTa-base BARNEY, to observe the relative performance on single-sentence classification.


% \input{tables/barney_training_ablation}

% For classification, we observe that... \ivan{Preliminary experiments show Denoising, Fixed performs best}

% For generation, we observe that....

% \ivan{The following are parameters to do ablation studies on their effect on classification and generation: The different training methods, the number of decoder layers, the amount of attention heads in the bottleneck, the effect of the gating method}


% \subsection{Context Attention Bottleneck Heads}
% To evaluate the importance of the number of heads in the context attention bottleneck, we finetune BERT with the Context Attention Bottleneck on a combination of the SNLI (\url{https://www.aclweb.org/anthology/D15-1075.pdf}) and Multi-Genre NLI (\url{https://www.aclweb.org/anthology/N18-1101.pdf}) datasets and evaluate the the Spearman correlation of the cosine similarity between sentence embeddings on the STS benchmark test set

% \subsection{Semantic Textual Similarity}
% \ivan{Here, we can run the semantic textual similarity benchmark as in the SentenceBERT paper (Train on AllNLI, eval on STS) \url{https://arxiv.org/pdf/1908.10084.pdf}, first by just plugging in our bottleneck and comparing scores to show our bottleneck is better than simply summing/averaging/maxing the contextualized representations. We can then show a plot on how (for a fixed seed) the score changes as we vary the amount of heads in the bottleneck}
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c}
%         \textbf{Model} & \textbf{Spearman}  \\
%         \hline
%         Avg. GloVe embeddings & 58.02  \\
%         Avg. BERT embeddings & 46.35  \\
%         InferSent - GloVe & 68.03  \\
%         Universal Sentence Encoder & 74.92 \\
%         SBERT-NLI-base & 77.03 \\
%         SBERT-NLI-large & 79.23 \\
%         BARNEY-bert-base h=6 & TBD \\
%         BARNEY-bert-base h=12 & TBD \\
%         BARNEY-bert-base h=24 & 0.7423 \\
%         BARNEY-bert-base h=48 & 0.7400 \\
%         BARNEY-bert-base h=96 & 0.7357 \\
%         BARNEY-bert-base h=192 & 0.7389 \\
%         BARNEY-bert-base h=384 & 0.7421 \\
%         BARNEY-bert-base h=768 & 0.7343 \\
%         BARNEY-bert-large h=X & TBD \\
%     \end{tabular}
%     \caption{Evaluation of the Spearman correlation of the cosine similarity of sentence embeddings on the STS benchmark test set for models trained on the combination of the SNLI (\url{https://www.aclweb.org/anthology/D15-1075.pdf}) and Multi-Genre NLI (\url{https://www.aclweb.org/anthology/N18-1101.pdf}) dataset}
%     \label{tab:offsetablation}
% \end{table}
% \ivan{The above can be reduced to a plot}



% \ivan{They present results for "train NLI, eval STS", "train STS, eval STS", "train STS+NLI, eval STS"}

% \section{Results}
% Some preliminary training plots for training on 320k common crawl sentences: \\
% \textbf{TAE}: The following was obtained by using the base parameters specified in the original Attention is All You Need paper, along with the inverse square root learning rate annealing, and a hidden representation of 512. \\
% \includegraphics[width=.375\textwidth]{TAE.png} \\
% \textbf{BARNEY}: The following was obtained by using BERT (base-uncased) as the transformer encoder, projecting to a hidden representation of 512, and using a decoder identical to TAE. \\
% \includegraphics[width=.375\textwidth]{BARNEY.png} \\


==> sections-old/6-relatedwork.tex <==
\section{Related Work}
\nikos{let's remove this section and incorporate the citations throughout the text were relevant.}
\nikos{ These are some recent transformer papers related to autoencoders (none of them focuses on pretraining):} \\
- \url{https://www.ijcai.org/Proceedings/2019/0727.pdf}\\
- \url{https://arxiv.org/pdf/1809.11155.pdf} \\
- \url{https://arxiv.org/pdf/1905.02450.pdf} \\
- \url{https://arxiv.org/pdf/1908.10084.pdf} \\
- \url{https://www.ijcai.org/Proceedings/2019/0727.pdf}\\
\ivan{More papers to cite} \\
- \url{https://arxiv.org/pdf/2006.03236.pdf} \\
- \url{https://arxiv.org/pdf/1905.12926.pdf} \\
- \url{https://arxiv.org/pdf/1812.10464.pdf} \\
- \url{https://arxiv.org/pdf/1506.02216.pdf} \\

\ivan{Can bring a lot more references from the Emb2Emb paper}

==> sections-old/generation.tex <==
\begin{table}[]
\centering  
\footnotesize
\begin{tabular}{ll|cc} 
\toprule
\textbf{Model} &  & \textbf{ACC} & \textbf{BLEU} \\
\midrule
% \multirow{3}{*}{AAE} & $\pm v$ & 7.2 &	86.0 & 33.7 \\
%  & $\pm 1.5v$ & 25.1 &	59.6 &	59.5 \\
%  & $\pm 2v$ & 57.5 & 27.4 & 139.8 \\
% \hline
\multirow{3}{*}{DAAE} & $\pm v$ & 36.2 & 40.9 \\
 & $\pm 1.5v$ & 73.6 & 18.2 \\
 & $\pm 2v$ & 91.8 & 7.3 \\
\hline
\multirow{3}{2cm}{AUTOBOT roberta-base} 
 & $\pm 0v$ & 8.4 & 45.10  \\
 & $\pm v$ & 22.8 & 39.78 \\
 & $\pm 2v$ & 55.4 & 26.83 \\
 & $\pm 3v$ & 79.3 & 15.08  \\
 & $\pm 4v$ & 87.8 & 7.41  \\
\hline
\multirow{3}{2cm}{AUTOBOT roberta-base ft3} 
 & $\pm 0v$ & 5.3 &  83.60 \\
 & $\pm v$ & 6.5 & 80.69 \\
 & $\pm 2v$ & 14.1 & 68.36 \\
 & $\pm 3v$ & 40.9 & 43.46  \\
 & $\pm 4v$ & 69.7 & 21.70  \\
 & $\pm 6v$ & 91.9 & 4.46 \\
\hline
\multirow{3}{2cm}{AUTOBOT roberta-base ft1} 
 & $\pm 0v$ & 6.1 & 75.22 \\
 & $\pm v$ & 10.7 & 69.51 \\
 & $\pm 2v$ & 35.0 & 51.91 \\
 & $\pm 3v$ & 69.4 & 25.53  \\\hline
\multirow{3}{2cm}{AUTOBOT roberta-base full} 
 & $\pm 0v$ & 7.9 & 60.34  \\
 & $\pm v$ & 20.4 & 59.54 \\
 & $\pm 2v$ & 50.3 & 41.47  \\
\hline
% \hline
% \multirow{3}{2cm}{BARNEY-base l1} 
%  & $\pm 0v$ & 8.3 & 49.67  \\
%  & $\pm v$ & 23.6 & 43.37  \\
%  & $\pm 1.5v$ &  &   \\
%  & $\pm 2v$ & 54.8 & 28.94  \\
% \hline
% \multirow{3}{2cm}{BARNEY-base l1 ft1} 
%  & $\pm 0v$ & 6.25 & 76.76  \\
%  & $\pm v$ &  & 71.80   \\
%  & $\pm 1.5v$ &  &   \\
%  & $\pm 2v$ &  & 54.60  \\
% \hline
% \multirow{3}{2cm}{BARNEY-base l1 ft2} 
%  & $\pm 0v$ & & 82.46 \\
%  & $\pm v$ &  & 80.68 \\
%  & $\pm 1.5v$ &  &  \\
%  & $\pm 2v$ &  & 69.83 \\
% \hline
\multirow{3}{2cm}{BARNEY-large} 
 & $\pm v$ &  &		 \\
 & $\pm 1.5v$ &  &   \\
 & $\pm 2v$ &  &  \\\bottomrule
\end{tabular}  
%\vspace{-5pt}
\caption{
Automatic evaluations of vector arithmetic for sentiment transfer: Plotted as Accuracy vs. Self-BLEU.
Accuracy (ACC) is measured by a sentiment classifier, and values for varying multiples of the sentiment vector are plotted. Upper right is better.

% \nikos{add efficiency column that compares speed, add more tables from pnp autoencoder paper. remove ppl if the results are not calculated with the same vocab}

}\label{tab:res_sentiment}
%\vspace{-5pt}
\end{table}  

==> sections-submission/0-abstract.tex <==

\begin{abstract} %  


% Revised version from Noah's version
Representation learning for text via pretraining a language model on a large corpus has become a standard starting point for building NLP systems.  This approach stands in contrast to autoencoders, also trained on raw text, but with the objective of learning to encode each input as a vector that allows full reconstruction.  Autoencoders are attractive because of their latent space structure and generative properties. We therefore explore the construction of a sentence-level autoencoder from a pretrained, frozen transformer language model. We adapt the masked language modeling objective as a generative, denoising one, while only training a sentence bottleneck and a single-layer modified transformer decoder.
We demonstrate that the sentence representations discovered by our model achieve better quality than previous methods that extract representations from pretrained transformers on text similarity tasks, style transfer (an example of controlled generation), and single-sentence classification tasks in the GLUE benchmark, while using fewer parameters than large pretrained models.\footnote{Our code is available at: \url{https://github.com/ivanmontero/autobot}} 



% % Noah's 5/10 version with comments
% Representation learning for text via pretraining a language model on a large corpus has become a standard starting point for building NLP systems.  This approach stands in contrast to autoencoders, also trained on raw text, but with the objective of learning to encode each inputs as a vector that allows full reconstruction.  Autoencoders are attractive because of their generative latent space properties. We therefore explore the construction of a sentence-level autoencoder from a pretrained, frozen transformer language model. We adapt the masked language modeling objective as a generative, denosing one, We demonstrate that the sentence representations discovered by our method are a \nascomment{nail down claims about effiency, it's not clear to me right now} and perform competitively with the state of the art \nascomment{check that claim!} on text similarity tasks, style transfer (an example of controlled generation), and sentence classification tasks in the GLUE benchmark.

% \nascomment{fill this in}. (to keep computational cost low) 

% \nascomment{one thing not clear from the paper and possibly worth raising even here:  what data gets used to learn the autoencoder?  also, we need to nail down terminology.  in some places you say that the autoencoder is ``pretrained'' but I think that's confusing since we start from a pretrained model.  do we want to say that we finetune the autoencoder?} 


% old version commented out 5/10 by Noah
%Methods for obtaining unsupervised language representations have gained much attention recently for their performance on downstream tasks, and have largely relied on partial reconstruction of the input though masked language modeling or next token prediction through language modeling.
%Autoencoders, trained on full reconstruction of the input through a single fixed length, bottlenecked representation, have not been extensively studied for pretraining sentence-level representations, especially with transformers.
%To this end, we propose \textsc{Autobots}, a new class of text autoencoders with a sentence bottleneck derived from pretrained transformers on unlabeled data.
%Our training objective is to reconstruct sentences fully from a learned bottleneck representation while keeping the underlying pretrained model fixed.
%We demonstrate that the resulting sentence representations outperform previous methods on text similarity tasks while being parameter efficient, and can also be used for controlled generation tasks such as style transfer.
%Notably our method maintains the performance of the pretrained language model on other supervised  downstream tasks.







% Pretrained language models based on transformers have been shown to produce sub-optimal sentence representations for tasks requiring text similarity \cite{Reimers2019SentenceBERT}.
% Previous methods that ameliorate this issue have introduced auxiliary sentence similarity objectives that rely on annotated data and compose sentence representations with non-parametric pooling that exhibits limited desirable properties and is specific to text similarity tasks.
% To this end, we propose \textsc{Autobots}, a new class of text autoencoders with a sentence bottleneck derived from pretrained transformers on unlabeled data.
% Our training objective is to to reconstruct sentences fully from a learned bottleneck representation as opposed to partially from variable-length representations in existing masked language modeling objectives.
% We demonstrate that our resulting sentence representations outperform previous methods on text similarity tasks while being parameter efficient, and can also be used for controlled generation tasks such as style transfer.
% Notably our method maintains the performance of the pretrained language model on other supervised  downstream tasks.

% \nikos{new take on the abstract, please check. I tried to emphasize on the sentence BERT method to have a clear message about our goal of the paper. There are some nice points in the previous abstract that should probably be incorporated in the introduction but it would be crucial not to make big claims about pretraining in general since it would be hard to compete with big LM papers. }


% ===== nikos =====
% Pretrained language models based on transformers have been shown to produce sub-optimal sentence representations for tasks requiring text similarity \cite{Reimers2019SentenceBERT}.
% Previous methods that ameliorate this issue have introduced auxiliary sentence similarity objectives that rely on annotated data and compose sentence representations with non-parametric pooling that exhibits limited desirable properties and is specific to text similarity tasks.
% To this end, we propose \textsc{Autobots}, a new class of text autoencoders with a sentence bottleneck derived from pretrained transformers on unlabeled data.
% Our training objective is to to reconstruct sentences fully from a learned bottleneck representation as opposed to partially from variable-length representations in existing masked language modeling objectives.
% We demonstrate that our resulting sentence representations outperform previous methods on text similarity tasks while being parameter efficient, and can also be used for controlled generation tasks such as style transfer.
% Notably our method maintains the performance of the pretrained language model on other supervised  downstream tasks.
% =================





% Methods for obtaining unsupervised language representations have gained much attention recently for their performance on downstream tasks, and have largely relied on partial reconstruction of the input though masked language modeling or next token prediction through language modeling. Autoencoders, trained on full reconstruction of the input through a single fixed length, bottlenecked representation, have not been extensively studied for pretraining sentence-level representations, especially with transformers.
%In this paper, we propose the \textit{Transformer Autoencoder} by converting the architecture of \citet{vaswani17} to an autoencoder that uses attention to bottleneck the input to a single, fixed vector from which the input can be fully reconstructed. Leveraging the encoder advancements of \citet{devlin-etal-2019-bert}, we introduce \textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, and demonstrate the significant performance of this novel pretraining objective in downstream classification, sentence representation, reconstruction, and controlled generation tasks.

\end{abstract}

% Autoencoders have 

% Unsupervised pretraining has gained much attention recently 
% We propose the transformer

% Methods for obtaining unsupervised language representations have gained much attention recently for their performance on downstream tasks, and have largely relied on partial reconstruction of the input though masked language modeling or next token prediction through language modelling.

% Text autoencoders obtain an unsupervised sentence-level representation by bottlenecking with reconstruction abilities, but largely rely on recurreence in the decoder.

% In this paper, we propose the \textit{Transformer Autoencoder} model by converting the architecture of \citet{vaswani17} to an autoencoder that uses attention to bottleneck the input to a single, fixed vector from which the input can be fully reconstructed. Leveraging the encoder advancements of \citet{devlin-etal-2019-bert}, we introduce textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, to demonstrate the performance of this novel pretraining objective in downstream classification, sentence representation, reconstruction, and controlled genration tasks.

% by leveraging the encoder advancements of \citet{devlin-etal-2019-bert} in a transformer auto


% effectively enriching the resulting sentence representations with reconstructive properties. Concretely, we introduce a context attention bottleneck after the original encoder, and a modify the decoder to perform full reconstruction of the input conditioned on the bottleneck representation.
 
% Currently langauge representat
% 
 

% VERSION 1:

% % to learn 
% % \textit{BERT isn't an autoencoder, but BARNEY is!}

% Autoencoders have gained much attention for their unsupervised ability to reduce variable length sequences to a single latent space with reconstruction capabilities, yet current architectures rely heavily on recurrence. Similar to autoencoders, current state-of-the-art pretrained transformer models produce variable-length token represenations by learning to partially reconstruct their input, yet rely on a special token to produce sentence representations for most downstream natural language understanding tasks requiring a single vector.


% % Current state-of-the-art pretrained language models produce variable-length token representations by learning to partially reconstruct the input, and rely on a special token to produce sentence representations for most downstream natural language understanding tasks requiring a single vector. 
% %\nikos{we may want to mention that it's not possible to produce the full sentence based on cls alone} 
% %\nikos{the token level representations are used for word-level tasks though, so we have to make sure we don't overclaim here.}

% In this paper, we propose the \textit{Transformer Autoencoder} model that results from  converting the architecture of \citet{vaswani17} to an autoencoder that projects the input to a single, fixed vector from which the input can be fully reconstructed, effectively enriching the resulting sentence representations with reconstructive properties. 
% Concretely, we introduce a context attention bottleneck after the original encoder, and a modify the decoder to perform full reconstruction of the input %(instead of partial) 
% conditioned on the bottleneck representation.
% %to the "encoder-decoder" layer in the decoder stacks.
% %
% %We preserve the parallelism in the original transformer by analyzing dot-product attention's decomposition in the many-to-one and one-to-many settings. \nikos{Not sure I fully get this point. }
% %
% %\textbf{TAE} can be pre-trained on unlabeled corpora to produce a single sequence-level representation. \nikos{this point could be skipped}

% % Lastly, we develop an example framework called \textbf{BARNEY} based on transformer autoencoders for pretraining akin to BERT \citet{devlin-etal-2019-bert}
% Lastly, we introduce \textbf{BARNEY}, which stands for \textbf{B}ERT \textbf{A}ggregated \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}, which both leverages advancements of \citet{devlin-etal-2019-bert} and introduces a novel pretraining objective for transformers. We evaluate its sentence representations on downstream classification, reconstruction and controlled generation tasks.\footnote{Our code will be made available at [link]} 


% %, which stands for \textbf{B}idirectional \textbf{A}ggregated Transformer \textbf{R}epresentations by Reduci\textbf{n}g and R\textbf{e}constructing Full\textbf{y}. \nikos{is it ok if we skip the abbreviations until we decide the proper framing?}
% % and  we evaluate its sentence representations on downstream classification, reconstruction and controlled generation tasks.\footnote{Our code will be made available at [link]} 

==> sections-submission/1-introduction.tex <==
% {\color{red}TODOS
% \begin{itemize}
%     \item Ivan: Finalize tables, experiments, and figures, then work on text
%     \item Ivan $\&$ Nikos: Related Work \nikos{let's incorporate everything in the introduction. dedicating a whole section for this does not make much sense for a short paper.}
% \end{itemize}
% }



\section{Introduction} 

%\nikos{need to convert to full text}
%{\textit{Contributors}}: Ivan, Nikos, Noah

%\vspace{3mm} 
%\noindent \textit{Significance:} 
Recent research has focused on devising new unsupervised pretraining methods from unlabeled data that involves some form of language modeling, primarily autoregressive \citep{peters-etal-2018-deep,radford2019language}, masked \citep{devlin-etal-2019-bert, liu2019RoBERTa, conneau2020unsupervised} and generalized \citep{radford2019language, brown2020language,pmlr-v97-song19d}, with much success on downstream tasks.  Under the hood, most of these methods use transformers \citep{vaswani17} for encoding text sequences, which allows them to learn powerful contextual word representations that have been used widely for building models in NLP. However, this  does not hold for sentence representations derived from pretrained transformer language models based on a special token or basic pooling operations. In fact, previous studies have shown  that such sentences representations are sub-optimal for sentence similarity and  classification tasks. To this end, representation learning methods have been designed to better capture semantic information from pretrained transformer language models e.g.~ using Siamese networks trained with a triplet loss \cite{Reimers2019SentenceBERT} or transforming the desired sentence distribution to a Gaussian distribution through normalizing flows \cite{li-etal-2020-sentence}. 

Existing sentence representations directly derived from pretrained language models or learned by specialized methods cannot guarantee perfect reconstruction of the input, a property that can enhance the structure of their semantic space and enable their use for controlled generation tasks. For the latter, a few recent studies have looked into ways to steer generation of pretrained language models towards a particular style \citep{Dathathri2020Plug,krause2021gedi}, although they require following the gradient during the sampling process and rely on style text classifiers which might not be always available. The latent space of a text autoencoder allows one to perform controlled text generation through manipulating directly sentence representations using basic numerical operations \cite{pmlr-v119-shen20c}. Yet, how to convert pretrained transformer language models to autoencoders with such properties still remains unexplored. 

%as variable-length denoising has been explored \citep{lewis2019bart}. 
%Surprisingly, the direction of creating a complete autoencoder-like pretraining objective for transformers, where intermediate representation is of fixed size, still remains largely unexplored. 
% \citet{lewis2019bart} perform denoising, but accept a variable length hidden size from the encoder to the decoder. 
%\noindent \textit{Problem}:
% \nikos{here we need also to highlight the issue that was identified for sentence representations extracted from BERT in the SBERT paper and cite several studies that focus on sentence representations. By the way, do we have any comparison with other methods than SBERT? In that paper, they compare with other methods. Could we also compare with those?}
% (BERT, ELECTRA)
%Moreover, they produce variable-length token representations which are often not needed for the downstream tasks and are potentially redundant. 
%Additionally, during masked language modeling, only select tokens are updated each gradient step, encompassing wasted computation.
%To our knowledge, transformers decoders have not been explored in the context of a single encoder representation as input. \\
% \ivan{The [CLS] token, for BERT, is trained on the NSP task, which isn't sufficient for single-sentence representations. Additionally, in RoBERTa, they simply drop the NSP task altogether}

%\ivan{The two goals of this architecture: Improve BERT pretrained sentence representations, and provide a novel autoencoder (with better reconstruction properties)} 
% \vspace{3mm} 

% \noindent \textit{Questions}:
% \begin{enumerate}
%     \item Can we train BERT with a bottleneck representation from which the full input can be reconstructed?
%     \item How well will such representations perform on different tasks compared to the [CLS] token from BERT?
%     \item Will this autoencoder produce a latent representation that will do better on controlled generation tasks?
%     \item Can we obtain better token representations from BERT when pretraining on both the MLM and reconstruction objective?
%     %\item What do we want to make the scope of this paper be?
%     %\item Will this autoencoder do well in multilingual settings?
% \end{enumerate}

% \vspace{3mm}

%\noindent \textit{Method}:
% \nikos{a class of models for...} 
To fill in this gap, we introduce \textsc{Autobot}, a new autoencoder model for learning sentence bottleneck representations from pretrained transformers that is useful for similarity,  generation, and classification, displayed in Figure~\ref{fig:model}. Our model has two unique components: (i) a  transformation that uses dot product attention to dynamically pool semantic information from the pretrained model's hidden states into a sentence bottleneck representation, and (ii)  a shallow transformer decoder that is modified to operate based on the bottleneck representation. Instead of training our autoencoder from scratch, we directly finetune it using an input reconstruction objective on the unlabeled data on which the original pretrained transformer was trained. We keep the underlying pretrained transformer encoder fixed, which makes it more efficient than training from scratch
% \nascomment{reworked here, sentence was too long and some parts were misplaced}
% The additional computational overhead is 
%\nikos{can we make a comment here about the efficiency of this finetuning approach? how long does it take?} 
% \nikos{marginal? or mention percentage if available}
% marginal \nascomment{make quantitative} \nikos{number of steps divided by the number of steps in Roberta = ~20\%, we could say it takes 1/5 of the time it takes to train from scratch.} \ivan{part of the consideration here is that we don't need to back propgate into Roberta during finetuning, which is where the most speed gain we get comes from}
% compared to the total  time to required to pretrain
% \nascomment{pretrain?}
%  let’s remove marginal and mention that is more efficient than training from scratch because main model is kept frozen
% from scratch 
and proves beneficial even if we compare to pretrained transformers trained for an equal amount of steps. 

Our evaluation on representative sentence similarity, classification and generation tasks demonstrates that the   resulting sentence representations are compact, better capture semantic similarity at the sentence-level than strong sentence representation methods \cite{Reimers2019SentenceBERT} and can be used for controlled generation tasks.  Lastly, our model performs almost on par with the large RoBERTa model \citep{liu2019RoBERTa} even though it only introduces 1.6$\%$ additional
% \nascomment{make quantitative, e.g., a percentage} 
parameters relative to the base RoBERTa model. 

% \nikos{what about the experiments where we finetune some of the layers of the pretrained encoder? please clarify. } \ivan{they were only used in generation (figure 2), but it's a question if we want to include them or not (and make everything strictly using a fixed encoder).The current setup of the paper doesn't not include them}

% \nikos{ is it always the case that the pretrained encoder is fixed and what do we gain from this objective? }
% \textsc{autobots} use these components to perform full reconstruction of the input with a single, fixed length 
% which together are trained to perform full reconstruction of the input which is conditioned on the bottleneck representation.
% We fix the under
% As a use case we develop a language model pretraining framework based on our autoencoders akin to BERT. 
 
%\noindent \textit{Evaluation} 

% \nikos{let's make sure we include all the experimental details in the supplementary material (following emnlp guidelines) plus qualitative examples for all tasks that we examine.}
 %\ivan{Perhaps on reconstruction ability as well?}
 
%  \nikos{these contributions could be merged with the second to last paragraph above.}
% \noindent We summarize our contributions as:
% \begin{itemize}
%   \item \textsc{AUTOBOTS}: A new class of text autoencoders with a sentence bottleneck derived from pretrained transformers
%   \item An analysis of \textsc{AUTOBOTS} performance gains on single-sentence representation, generation, and classification tasks.
% \end{itemize} 

% \nikos{Please cite / discuss some of the most relevant ones in the end of second paragraph (before "To our knowledge").}
% \ivan{Papers to incorporate into introduction, mostly on autoencoding} \\

% - \url{https://www.ijcai.org/Proceedings/2019/0727.pdf}\\
% - \url{https://arxiv.org/pdf/1809.11155.pdf} \\
% - \url{https://arxiv.org/pdf/1905.02450.pdf} \\
% - funnel \url{https://arxiv.org/pdf/2006.03236.pdf} \\

% - \url{https://arxiv.org/pdf/1506.02216.pdf} \\
% - \url{https://arxiv.org/pdf/1812.10464.pdf} \\
% \nikos{ These are some recent transformer papers related to autoencoders (none of them focuses on pretraining):} \\



% \textit{Plan:}
% \begin{enumerate}
%     \item Classification tasks: We will primarily look into the GLUE framework to see what improvements BARNEY offers over BERT for classification, and see (using NLI/STS) its performance at creating sentence representations.
%     \item Generation tasks: We will evaluate on the Shen et. al. task to evaluate the generation capabilities of BARNEY and how it does as an autoencoder.
% \end{enumerate}

% \\
% \ivan{TODO List: \begin{enumerate}
%     \item Discuss the method more
%     \item Show the tables we would like to express, and what results we want to see.
% \end{enumerate}}
%\section{Context}
% Attention is All You Need \\
% RNN Autoencoder: \\
% Can get metrics in a multilingual setting (LASER): https://arxiv.org/pdf/1812.10464.pdf \\
% BERT: \\

% Can evaluate on all the tasks for reconstruction in emb2emb, and add classification on top. Emb2emb already contains everyting needed to evaluate

% Tasks can be multilingual (use multilingual BERT, eval against LASER)


==> sections-submission/2-proposedmethod.tex <==

\section{Model: \textsc{Autobot}}\label{sec:model}
% \nikos{Write a short sentence to summarize the key idea of the model and state that we take inspiration from relevant research  research on text autoencoders (+ cite a key one)}
%Our model aims to pool the variable-length pretrained transformer language model representations into a single, sentence-level representation with reconstructive capabilities. 
Taking inspiration from recent research on text autoencoders \citep{bowman2015generating,shen2019educating,mai2020plug}, we extend standard autoregressive text autoencoders, which have been predominantly based on recurrent networks, to a transformer-based architecture and integrate them with pretrained language models; here we focus on RoBERTa \cite{liu2019RoBERTa}.

%\nikos{Introduce here the basic formulation of autoencoders and keep only the novel parts in the following subsections}
Autoencoders generally follow the encoder-decoder model structure to reconstruct their input with the constraint that the encoder produces a single, fixed-length hidden representation $\text{enc}(\boldsymbol{x}) = \mathbf{z}$:
\begin{equation}
\text{AE}(\boldsymbol{x}) = \text{dec}(\text{enc}(\boldsymbol{x})) = \boldsymbol{x}'.
\end{equation}
\noindent Here, we focus on denoising autoencoders that aim to reconstruct a perturbed version of the input  \citep{vincent2010stacked,shen2019educating}, which is compatible with many of the pretrained language models that are based on masked language modeling. 
\subsection{Encoder}
\begin{figure}[ht]
\centering
\hspace{-2mm}\includegraphics[width=0.4\textwidth]{figures/autobots} 
\caption{\label{fig:model} % \nikos{new take}
Our autoencoder consists of a pretrained transformer encoder $\text{enc}$, a function $\beta$ that compresses the encoder's  final representations $\mathbf{H}$ of size $T \times d$ 
% \nascomment{need to give dimensions, you're assuming the reader will infer this is a matrix whose size depends on the number of words}
to a sentence bottleneck representation $\mathbf{z}$ of size $d$, and a transformer decoder $\text{dec}$ that is trained to fully reconstruct the training sentence $\boldsymbol{x}$. }
% \nikos{+1, I would keep it minimal and relatively small to save space e.g. even simpler than \url{https://paperswithcode.com/media/methods/Autoencoder_schema.png} perhaps with some indication that the encoder is a pretrained transformer.}}
% \caption{\label{fig:overview} We propose a novel task setup to multilingual question answering. A high resource language (HRL) question-answer database is leveraged by mapping a low resource language (LRL) query to a query in the database, then generating the LRL answer from the HRL answer.} % We examine using multilingual paraphrase detection in exploring the most reliable method to transfer knowledge from multilingual queries to English.
\end{figure}Standard approaches use encoders that reduce the input to a single representation $\mathbf{z}$. To use a pretrained transformer for this purpose we need to reduce its output hidden representations $\mathbf{H}$ after processing the input to a single vector. Since using the special token representation or basic pooling methods have been shown sub-optimal in prior work \cite{Reimers2019SentenceBERT}, here we opt to keep the original encoder fixed and train a transformation $\beta$ that will learn to compress $\mathbf{H}$ into a single representation   $\mathbf{z} = \beta(\mathbf{H}; \mathbf{\theta})$, with $\theta$ being an additional set of parameters to be learned during finetuning. We choose $\beta$ to be a multi-head attention mechanism that takes as input the keys  $\mathbf{K}$ and values $\mathbf{V}$ corresponding to the final representations $\mathbf{H}$ from the pretrained model
% \nascomment{confusing here:  all layers?  the last one?}
and a query vector $\mathbf{q}$ corresponding to a context vector $\mathbf{u}$ that we choose to be the \texttt{CLS} vector from the pretrained model:
%
\begin{align}
   \beta(\mathbf{H}; \mathbf{\theta}) &= \text{MultiHead}(\mathbf{q}, \mathbf{K}, \mathbf{V}) 
\end{align}
%
\noindent where the parameters to be learned, $\theta$, include the weights that are used to transform the query, keys, and values which amount to $ 3 d^2 $ with $d$ being the dimensionality of each head ($d = 64$ in our experiments).
% \nascomment{($d =$ (fill in) in our experiments)}. 

% \nikos{new simplified version above}
%\subsubsection{Sentence Bottleneck} 
%The Transformer encoder architecture outputs a hidden representation $\mathbf{h_t}$ for each input token $x_t$. We wish to reduce these representations to a single, fixed representation $\mathbf{z}$. The self-attention layers used in Transformers produce a many-to-many representation by making the keys, queries, and values come from the same input. In order to produce a many-to-one final representation, we introduce a context vector $\mathbf{u}$ to replace the query. 
% \ivan{I commented out option (1), which we could explore later, option (2) boils down to multihead attention with nhead=1, which we can examine in an ablation study}
%\begin{align*}
%    \mathbf{z} &= \text{SB}(\mathbf{u}, \mathbf{K}, \mathbf{V}) \\
%    &= \text{MultiHead}(\mathbf{u}^\top, \mathbf{K}, \mathbf{V}) \\
%       &= \text{Concat}(\text{head}_1, ..., \text{head}_n) \\%\mathbf{W_C} \nikos{is this transformation needed?}
%      \text{head}_i = & \text{Attention}(\mathbf{u}^\top \mathbf{W^{(i)}_Q}, \mathbf{K} \mathbf{W^{(i)}_K}, \mathbf{V} \mathbf{W^{(i)}_V})
%\end{align*} 

%\subsubsection{Pretrained transformers} 
% \nikos{should also mention here the finetuning options} 

%Let $\text{TE}(x)$ be an arbitrary transformer encoder and $\text{SB}(x)$ be the Sentence Bottleneck specified above. Then, the encoder of our transformer autoencoder is defined as the following. $$\mathbf{z} = \text{Enc}(\mathbf{x}) = \text{SB}(\mathbf{u}, \text{TE}(\mathbf{x}), \text{TE}(\mathbf{x}))$$ The context vector $u$ can be either be represented as a learned parameter, or a pooling of the $\text{TE}(\mathbf{x})$. This context vector could additionally used to condition on different contexts to adapt a particular bottleneck to different types of information. 

% For \textsc{AUTOBOTS}, we choose $\mathbf{u}$ to be learned through the $\texttt{CLS}$ representation.

\subsection{Decoder}

The %"encoder-decoder attention" 
cross-attention layer in the Transformer decoder architecture by \citet{vaswani17}  expects hidden representations for every token input from the encoder in order for each output candidate to attend to each input token. In the situation where only a single representation comes from the encoder, we have
% Analyzing the self attention in the context of \textbf{TAE}, both the memory keys and values in the self attention come from the single hidden representation $z$, which reduces to simply the linear transformation of the latent representation of the input sequence for each output candidate. \ivan{Using the notation in the original paper, the derivation would be the following:}
\begin{equation}
    \text{Attention}(\mathbf{Q}, \mathbf{z}^\top \mathbf{W}_K, \mathbf{z}^\top \mathbf{W}_V) = \mathbf{z}^\top \mathbf{W}_V
\end{equation}
% \nascomment{changed $\mathbf{W_V}$ and similar to $\mathbf{W}_V$ and similar, note the difference}
%\nikos{ I don't get this. why the queries are ignored? isn't like doing cross-attention with a single token as source?} \ivan{Correct, so since this is the cross-attention layer, "queries" are the the current hidden states of the decoder. In other words, every timestep of the decoder will pull the exact same $\mathbf{z}^\top \mathbf{W_V}$ regardless of the current timestep}\nikos{hmm, then we could simply say that every query attends to the same sentence representation z instead of each token representation in the source sentence. saying that queries are ignored is a bit confusing.  }
Note that the queries $\mathbf{Q}$, which come from the previous masked self-attention layer, are not  taken into account, and each step in the decoder will receive the exact same $\mathbf{z}^\top \mathbf{W}_V$ as a result.  In order to mitigate this, we propose a gating method inspired by \citet{hochreiter1997long}. %\nikos{nice!}  
%  to allow the input query to control the per-element amount of information to include from the hidden representation vector
Concretely, let $\mathbf{Q_t}$ be the $t$th query representation. Then, the $t$th output $\mathbf{o}_t$ of the %"encoder-decoder"
cross-attention layer is computed as follows 
\begin{equation}
    \mathbf{g}_t = \sigma(\mathbf{G}  \mathbf{Q}_t + \mathbf{G'}  \mathbf{z});\ \  
        \mathbf{o_t} = \mathbf{g}_t \odot \mathbf{z}^\top\mathbf{W}_V
\end{equation}
% \nikos{the gate $g_t$ doesn't look at the \mathbf{z} vector at all, so it's output will be independent of the z vector. we should probably add z as input to make sure features from both $h_t$ and $z_t$ are considered. e.g. $W_g h_t + b_g + W_z z + b_z$}
\noindent where $\sigma(\cdot)$ is the \textit{sigmoid} activation function and $\mathbf{G}$ and $\mathbf{G}'$
%, $\mathbf{b_g}$ \nikos{let's suppress the biases for brevity}
are the parameters of the transformation for the gate. %\nikos{do we use different parameters here or it's one transformation for both Q and z?} \ivan{different parameters}
One can view the role of the gate as determining the amount of per-element information from the linear transformation of the latent representation to keep for the current layer and timestep.

\paragraph{Training considerations} To avoid training our model from scratch, we finetune it for 100K optimization  steps on a pretraining dataset using the base RoBERTa model \cite{liu2019RoBERTa} on the encoder side and a single layer 
% transformer \nascomment{this doesn't align with the decoder descirbed above which I don't think is a transformer}
decoder side for efficiency purposes \citep{kasai2021deep}. The model is trained using an input reconstruction loss by minimizing the negative log-likelihood computed over the reconstructed inputs. Note that only the parameters of the sentence bottleneck and the decoder are learned; the encoder parameters are kept fixed.

%Unlike the masked language modeling and next sentence prediction pre-training objectives of BERT, we introduce the unsupervised reconstruction objective by pairing \textsc{Autobots} with a transformer decoder and train on the task of reconstructing its own input. \nikos{this is already mentioned?}
%Previous work has shown denoising autoencoders provide better representations \cite{vincent2010stacked, shen2019educating}, so we use the masked language modeling input and task the decoder with producing the entire, unmasked sequence.
%We propose keeping BERT fixed throughout this process, and learning a representation from the final, fixed BERT output.
% Below are the methods that consider both fixed and trainable BERT:

% \subsubsection{Fixed BERT}
% One can use the fixed weights from BERT, and only finetune the bottleneck of the encoder with the decoder. Inspired by the objective of preserving the BERT representations, this method experiences speed benefits from not needing to backpropogate into BERT. The two methods this can be applied to are the following:


==> sections-submission/3-experiments.tex <==

\section{Experiments}\label{sec:experiments}
To assess the quality of the sentence representations learned by our model we evaluate on sentence similarity (Section \ref{sec:sim}), classification (Section \ref{sec:clf}), and generation tasks (Section \ref{sec:gen}).

%\nikos{we need to be more specific here. what are the questions we would like to answer specifically or our hypothesis. make sure the points we make correspond to the claims that we make in the intro/abstract and are clearly stated.}
% For fair comparison, we pretrain \textsc{Autobots} on the same Wikipedia + BooksCorpus dataset from BERT. To avoid training from scratch we use the pretrained BERT model as a starting point for our encoder function. We consider several different methods of pretraining. \nikos{these sound like experimental details, I would mention the basic ones in a subsection here and defer the rest for the supplementary (make sure we include everything there).}

\subsection{Settings} 
%\nikos{Add some basic details here. What data do we use + citation, where do we pretrain RoBERTa and for how long? fixed vs finetuning upper layers enc etc}
\paragraph{Datasets}
Since the RoBERTa dataset is not publicly available, we use for pretraining the exact same dataset as BERT \citep{devlin-etal-2019-bert}, which is composed of BooksCorpus \citep{zhu2015aligning} and English Wikipedia. For sentence similarity, we use the Natural Language Inference (NLI) dataset \citep{bowman2015snli} for finetuning and evaluate on the Semantic Textual Similarity (STS) dataset \citep{cer2017semeval}, following \citet{conneau2017supervised}.  For classification, we use mainly single-sentence datasets from the GLUE benchmark \citep{wang2018glue}, namely Stanford Sentiment Treebank (SST) and Corpus of Linguistic Acceptability (CoLA) datasets, but we also report the average performance on the remaining datasets. For generation, we use the Yelp reviews dataset \citep{shen2017style}.

% \nikos{we need to clarify if we use the exact same dataset and why. is it a subset of it or not?} \nikos{let's also mention here the details about datasets we use to evaluate each of the tasks for similarity, classsification and generation.}



% BooksCorpus (800M words) (Zhu et al.,
% 2015) and English Wikipedia (2,500M words). 
\paragraph{Baselines}
%\nikos{Mention which sentence representation methods we compare to (basic pooled, SBERT, etc) for each task.} 
For sentence similarity, we compare to SBERT which is a competitive method for deriving informative sentence representations from pretrained language models \cite{Reimers2019SentenceBERT}.\footnote{Note that, in contrast, our model does not require additional data during the pretraining phase. } They obtain sentence representations by using simple pooling methods over BERT representations such as mean and max (instead of the CLS token representation) and finetuning the whole pretrained model using Siamese networks and a triplet loss on a combination of natural language inference data.  To compare with them on sentence similarity, we incorporate our model within their framework and follow their settings and training/evaluation protocol (details in Appendix~\ref{adx:sentrep}). 

For sentence classification, we compare our model to RoBERTa-base and RoBERTa-large models \cite{liu2019RoBERTa}.  % They achieve sentence representations by encoding the premise $x$ and hypothesis $y$ sentences separately to get $\mathbf{z_x}$ and $\mathbf{z_y}$ respectively, then finetune a linear classification layer with softmax loss over the concatenation of $[\mathbf{z_x};\mathbf{z_y};|\mathbf{z_x}−\mathbf{z_y}|]$. \nikos{I feel this part can be skipped, is it that important to mention it in detail? Mentioned a high-level view of this.}

For sentence generation tasks, we compare to a strong and efficient style transfer method by \citet{shen2019educating}, which is a recurrent network-based denoising text autoencoder on in domain data. The style transfer is achieved  through vector arithmetic, namely computing a “sentiment vector” $\mathbf{v}$ by taking the vector difference between 100 negative and positive sentences, then evaluating by taking an input sentence, encoding it, adding a multiple of the sentiment vector to the sentence representation, then decoding the resulting representation. In addition to the denoising auto encoder (DAE) of \citet{shen2019educating}, we include more sophisticated methods for style transfer that are more computationally expensive such as fast gradient iterative modification (FGIM) of \citet{wang2019controllable} and Emb2Emb of \citet{mai2020plug} for reference.
 

% \nikos{Make clear on which tasks we finetune the whole model and which ones RoBERTa model is kept fixed. This is not clear at all up to this point.} \ivan{they were only used in generation (figure 2), but it's a question if we want to include them or not (and make everything strictly using a fixed encoder). The current setup of the paper doesn't not include them} \nikos{I meant when finetuning on a downstream task. regarding finetuning with the autoencoding objective we still need to mention what options we consider; hmm, yes let's describe everything and we decide after. }

% \subsection{BARNEY Pretraining for Classification}
% We outline several methods to pretrain BARNEY, and perform experiments on the sentence similarity task (SST2) with RoBERTa-base BARNEY, to observe the relative performance on single-sentence classification.

% \input{tables/barney_training_sst}

% \noindent \textbf{Datasets} \nikos{Mention some basic details about the datasets used here.}
% In our experiments
% NLI, GLUE, STS
 
% \noindent \textbf{Model configuration} \nikos{Only the basic ones and defer to the supplementary for the details such as number of epochs, learning rate etc. (e.g. we follow configuration from ...)}

% \noindent \textbf{Baselines} \nikos{Describe our baselines and the versions of our model that we examined.}



% \noindent \textbf{Datasets} \nikos{Mention some basic details about the datasets used here.}
% In our experiments
% NLI, GLUE, STS
 
% \noindent \textbf{Model configuration} \nikos{Only the basic ones and defer to the supplementary for the details such as number of epochs, learning rate etc. (e.g. we follow configuration from ...)}

% \noindent \textbf{Baselines} \nikos{Describe our baselines and the versions of our model that we examined.}


% \ivan{For each experiment, I will follow your Datasets, Model Configuration, Baselines format in the description}

\subsection{Sentence Similarity} \label{sec:sim}
%\nikos{you could mention the more general idea behind experiments in the first paragraph of this section and point to subsections (e.g. that we evaluate the representation and sentence generation quality of sentence representations extracted from pretrained models.}
% {
%\citet{conneau2017supervised} show that universal sentence representations can be obtained from finetuning on the NLI training data and evaluating the model's efficacy using the STS benchmark data. \nikos{Mentioned in the dataset section?} 

% The spearmen
 The results on the sentence similarity task are displayed in Table~\ref{tab:nli_sts}.
%  \nascomment{this reference is wrong, it refers to a section not a table; probably the label command isn't inside the table's caption?}. 
 We can observe that \textsc{Autobot} applied to RoBERTa-base significantly outperforms other base transformer methods. Additionally,  \textsc{Autobot} approaches the performance of large  transformers while having a minimal   parame-\input{tables/sts}   \input{tables/pooling} \noindent ter overhead of 1.6\%. Due to resource constraints and unreported results by prior work, we report our model only with RoBERTa-base.  % \nascomment{make this quantitative}. \nikos{done}
% \nascomment{maybe footnote this:}

% \nascomment{this is strange wording; do you mean that previous work didn't report it?}, we report our  model only applied to RoBERTa-base and leave the hyperparameter search required for large models to future work.
 
%  \nascomment{tables are perhaps ordered wrongly?  in the table currently numbered 2, mark which system(s) are ours.}
 

 
% We directly compare to the results of \citet{Reimers2019SentenceBERT} as well as 
% }\ivan{Finish
% We directly compare against finetuning the original pretrained versions of BERT and RoBERTa, as well as \citet{Reimers2019SentenceBERT}'s 
% \citet{Reimers2019SentenceBERT} perform the methodology of  by using simple pooling methods of BERT representations, such as mean, max, and cls, and evaluate their performance on sentence similarity task. We train and evaluate \textsc{Autobots} with a similar setup and its unique context attention bottleneck to compare against their results.
% \citet{conneau2017supervised} show that one can obtain universal sentence representations by finetuning on natural langauge inference data. \citet{Reimers2019SentenceBERT} show how this methodology can be applied to pooled BERT representations to obtain such sentence representations. We compaire
We find in Table~\ref{tab:pooling} that using the proposed sentence bottleneck based on learned context  provides 
% \nascomment{do not use this word if you're not doing hypothesis tests} significant 
noticeable gains over using simpler pooling methods from prior work. We suspect this is due to the additional flexibility provided by our bottleneck acting as ``weighted pooling'' by attending over all tokens to compute the final representation, as opposed to equal contribution of all tokens regardless of the input. 




% We also find it maintains same relative performance in the large transformer models. Due to resource constraints, we use SBERT's defaults leave further hyperparameter optimization of the large transformer models to future work.

% we compare directly the performance of \textsc{Autobots} to other models on the sentence similarity task, ones which have not been trained on STS data. We find that \textsc{Autobots} ends up performing singificantly better, and ends up achieving SBERT-large level performance with significantly less parameters.


\subsection{Sentence Classification} \label{sec:clf}

The results on single-sentence classification tasks and other tasks from the GLUE benchmark are displayed in Table \ref{tab:glue}. We find that \textsc{Autobot} provides a 
% \nascomment{do not use this word if there's no test} significant
noticable performance increase on single-sentence tasks, specifically on the CoLA datasets when using both the RoBERTa-base and RoBERTa-large models.
% This demonstrates that our model is effective regardless \nascomment{too strong; we only tested two model sizes!} of the pretrained language model's size used.
Additionally, we also find that \textsc{Autobot}, when fed both sentences concatenated for dual sentence GLUE tasks, maintains the original performance of the underlying pretrained encoder. Hence, our model improves the quality of the sentence representations from pretrained transformer models without hurting their performance.  

%The GLUE benchmark is a collection of diverse natural language understanding text classification, and involves both single and dual sentence tasks. 
%We fully finetune \textsc{autobots} single sentence tasks and compare performance with \citet{liu2019RoBERTa} in Table~\ref{tab:glue}. \nikos{moved them above}

% We evaluate \textsc{Autobots} pretrained with the Denoising, Fixed methodology report its performance on the dev set of each task in Table 1. \\
% We find that on multiple tasks \textsc{Autobots} on the base models end up performing on par with the large models with a mere fraction of additional parameters and compute. 

\input{tables/glue}

% \ivan{describe finetuning: fully finetuned autobots}
% \ivan{Should we include results where the final layers of the pretrained model are trainable? It would make figure 2 a bit more crowded}\nikos{let's add them in the supplementary section.}

% \ivan{Since these are classification tasks, I feel like BARNEY would have a good chance at beating BERT as a baseline. These classification task require backpropagation through BARNEY, in addition to the linear classification layer, in the finetuning process.}
% \nikos{We should definitely try this. I am curious to see how the autoencoder pretraining objective impacts the results. } 



% \subsection{SentEval}
% SentEval [cite] is an evaluation framework for fixed sentence embeddings on 17 downstream tasks. We follow a setup similar to \cite{Reimers2019SentenceBERT} by finetuning on a combination of Natural Language Inference and Semantic Textual Similarity training sets, then finetuning a linear regression head on the fixed representations for each task. We examine the perfomrance of both BARNEY and BERT + CAB.
% % \ivan{These are 17 downstream tasks that \textit{don't} backpropagate through the sentence encoder, but rather, evaluate the fixed-length sentence embeddings themselves. \url{https://github.com/facebookresearch/SentEval}. If we include BERT's [CLS] token in this framework, we definitely have a good shot here}
% \nikos{I don't believe that this evaluation will measure the full potential of the method since it's best on fixed embeddings. By the way some of these tasks overlap with GLUE where we plan to test anyway with finetuning (e.g.SST/MRPC). So, I'd rather suggest to look for some controlled generation task such as sentiment style transfer (e.g. like the one used by Shen et al 2020) to demonstrate the benefits for a real  generation task (other than the reconstruction tests below).}
% % \ivan{Gotcha. In SentenceBERT they test the fixed embeddings after finetuning to the NLI dataset, which I feel like a good table to include would be an extra row for our method on table 5: \url{https://arxiv.org/pdf/1908.10084.pdf}}


% \subsection{BARNEY Pretraining for Generation}
% We outline several methods to pretrain BARNEY, and perform experiments on the sentence similarity task (SST2) with RoBERTa-base BARNEY, to observe the relative performance on single-sentence classification.





% \subsection{Multilingual}

% \subsection{Pretraining}
% \begin{itemize}
%     \item Train two models on the exact same data for the exact same amount of training steps. To simulate the same amount of parameters, use one extra layer for the MLM approach
%     \item Model 1: 7 layer, 512 hidden size transformer encoder trained on just the MLM objective
%     \item Model 2: 6 layer, 512 hidden size BARNEY trained on MLM objective in conjunction with reconstruction objective.
%     \item Show the down-stream MNLI performance difference after certain amounts of steps (could be a plot)
%     \item Show the downstream SQuAD (MNLI?) performance difference at the end of BARNEY wihtout the conetext attention bottleneck (see if the reconstruction objective helps with better token-level representations, since all tokens are updated each step, rather than only 15\% of them in MLM)
% \end{itemize}

\begin{figure}[ht]
\vspace{-5.5mm}
\centering
\hspace{-2mm}\includegraphics[width=0.5\textwidth]{figures/generation_more_points.png}
\caption{ 
% \nikos{it'd be nice also to add some points from prior work (pnp paper models)?} \ivan{I'll try finding and adding some} 
% \nikos{great!} \nikos{the fontsize on legends, xticks, yticks, xlabel, ylabel still look quite small. }
% \nikos{could we remove two of the autobot models to make the diagram more clear? it'd be nice also to add some points from prior work (pnp paper models)? no need to have a line for these others. could you me the markers equal size and a bit bigger? I'd use a solid or dotted line without markers for the baseline.}
% \nikos{please also make font for the axes and their titles bigger. I'd also remove the top title from the figure, caption is sufficient and you save up space.}
Automatic evaluations of vector arithmetic for sentiment transfer, plotted as accuracy vs. self-BLEU. Accuracy (ACC) is measured by a sentiment classifier, and values for varying multiples of the sentiment vector are plotted. Upper right is better.
% \ivan{We also have examples where the last 3 layers of the pretrained transformer were allowed to be finetuned} \nikos{these results are without finetuning? yeah if it is very crowded we should include the ones with finetuning in the supplementary.  }\nikos{can we increase the font sizes a bit more and the thickness of the lines? I'd use dashes instead of dots for the baseline with thicker lines because it looks more distinctive.}
% \nikos{add efficiency column that compares speed, add more tables from pnp autoencoder paper. remove ppl if the results are not calculated with the same vocab}
\label{fig:generation}
}
\end{figure}
\subsection{Sentence Generation} \label{sec:gen}
% sentiment style transfer (e.g. like the one used by Shen et al 2020)
%\citet{mikolov2013linguistic} previously discovered that embeddings from unsupervised learning can capture linguistic relationships via simple arithmetic. \nikos{let's keep this for the longer version?}

% A canonical example is the embedding arithmetic “King” - “Man” + “Woman” $≈$ “Queen”.

%To evaluate latent space properties of autoencoders, \citet{shen2019educating} propose evaluating unsupervised style transfer through vector arithmetic computing a “sentiment vector” $v$ by taking the vector difference between 100 negative and positive sentences, then evaluating by taking an input sentence, encoding it, adding a multiple of the sentiment vector to the sentence representation, then decoding the resulting representation. \nikos{Moving it up}

% \nascomment{missing number in lower right of table 3 is not explained}

For sentence generation, we focus on the sentiment transfer task proposed by \citet{shen2019educating} both with and without further training on in-domain data from Yelp. When finetuning, we perform an additional 10K optimization steps using the Yelp dataset.  Note that all the baselines require training on in-domain data, while this is optional for our model.  In Figure~\ref{fig:generation}
% \nascomment{reference goes to a section not a figure}
we find that the \textsc{Autobot} model not exposed to the Yelp dataset during finetuning performed on par with the 
% \nascomment{DAE is not explained, either in the text or the figure -- reader doesn't know what it is}
DAE that was trained specifically on Yelp. Additionally, \textsc{Autobot} outperforms the DAE in the above-40 percent accuracy range when finetuned on in-domain data.
% \nascomment{what follows is a bit too vague.  either explain more fully or cut} Lastly, we additionally find that with partial finetuning of the pretrained transformer encoder \textsc{Autobot} achieves higher BLEU for a given accuracy, which we defer to the appendix.
We include \textsc{autobot} results with partial finetuning of the encoder in the appendix.
% \nascomment{there's no supplementary ... I think we referred to it as appendix before?}.
Since \textsc{AUTOBOT} uses vector arithmetic, inference is as fast as the DAE and over twice that of other methods.
% \nikos{say something about speed compared to previous methods}
% and compare directly with We compare directly with \citet{shen2019educating} and their denoising autoencoder (DAE) trained on Yelp, and include more sophisiticated methods for style transfer such as fast gradient iterative modification (FGIM) of \citet{wang2019controllable} and Emb2Emb of \citet{mai2020plug} for reference \citet{shen2019educating} and their denoising autoencoder (DAE) trained on Yelp. We evaluate \textsc{autobots}
% wang2019controllable

% , and explore the effect of making several last layers of the pretrained transformer trainable during autoencoding. 

% To evaluate properties of the latent space of \textsc{Autobots}, we perform the experiment of \citet{shen2019educating} were we compute a “sentiment vector” $v$ from 100 negative and positive sentences, and change the sentiment of a sentence by encoding it, adding a multiple of the sentiment vector to the sentence representation, then decoding the resulting representation.

% We plot the sentiment classification accuracy versus self-BLEU curve as we vary the multiple of the sentiment vector added used in .


% FGIM \citep{wang2019controllable} fast gradient iterative modification


% We also observe that when more of the final layers of the pretrained encoder are allowed to be finetuned with the autoencoding objective, \textsc{autobots} obtain higher Self-BLEU in the sub-90 percent accuracy range.

% \ivan{describe finetuning: fixed autobots evaluated}
% and use it to change the sentiment of the test sentences.

% \input{tables/generation}

% \subsection{Reconstruction Quality}
% \ivan{Perhaps we should evaluate the reconstruction ability compared to other autoencoders? We could focus on just BooksCorpus, create our own test set, and test reconstruction quality. If TAE/BARNEY is really good, we could introduce EM as a metric}
% \nikos{ What do you mean by EM? I worry that we may not have the space for introducing a new evaluation too (we have new architecture + pretraining framework already). How about using the Yelp dataset to compare directly with Shen et al 2020 in their own setup? }


% \subsection{Latent Properties}
% \ivan{We could also show an example of encoding two sentences, then showing the decoding of the linear interpolation of between the two? Perhaps a 2D dim-red of the embeddings?} \nikos{Sure, that'd be great. E.g. like the ones here \url{https://arxiv.org/pdf/1511.06349.pdf}}




==> sections-submission/4-conclusion.tex <==
\section{Conclusion}
% \ivan{make a conclusion}
%In this paper, we present \textsc{Autobots}, the construction of a sentence-level autoencoder from a pretrained, frozen transformer language model that adapts the masked language modeling objective as a generative, denoising one.
We proposed an approach that converts a pretrained transformer language model into a  
% \nascomment{I think ``standalone'' might be better than ``fully fledged''?  though I'm not sure standalone is accurate because we still need Roberta to do the encoding} \nikos{[right. perhaps, we could say "standard" or avoid specifying}
sentence-level autoencoder that is able to reconstruct its pretraining data. The resulting model improves the performance of the pretrained model on sentence-level tasks while maintaining its performance on multi-sentence tasks. In addition, the new sentence representations are suitable for efficient conditional text generation such as sentiment transfer without the need for training on in-domain data. 
% We, there-fore,  explore  the  construction  of  a  sentence-level  autoencoder  from  a  pretrained,  frozentransformer  language  model.    We  adapt  themasked language modeling objective as a gen-erative,  denoising  one,  while  only  training  asentence  bottleneck  and  a  single-layer  modi-fied  transformer  decoder.



% In this paper, we present Emb2Emb, a framework
% that reduces conditional text generation tasks to
% learning in the embedding space of a pretrained
% autoencoder. We propose an adversarial method
% and a neural architecture that are crucial for our
% method’s success by making learning stay on the
% manifold of the autoencoder. Since our framework
% can be used with any pretrained autoencoder, it
% will benefit from large-scale pretraining in future
% research.
